A Theory of Abstraction in Reinforcement Learning

Reinforcement learning defines the problem facing agents that learn to make good decisions through action and observation alone. To be effective problem solvers, such agents must efficiently explore vast worlds, assign credit from delayed feedback, and generalize to new experiences, all while making use of limited data, computational resources, and perceptual bandwidth. Abstraction is essential to all of these endeavors. Through abstraction, agents can form concise models of their environment that support the many practices required of a rational, adaptive decision maker. In this dissertation, I present a theory of abstraction in reinforcement learning. I first offer three desiderata for functions that carry out the process of abstraction: they should 1) preserve representation of near-optimal behavior, 2) be learned and constructed efficiently, and 3) lower planning or learning time. I then present a suite of new algorithms and analysis that clarify how agents can learn to abstract according to these desiderata. Collectively, these results provide a partial path toward the discovery and use of abstraction that minimizes the complexity of effective reinforcement learning.

==> algorithms/ac_dibs_alg.tex <==
% ----------
% -- AC-DIBS --
% ----------
\begin{algorithm}[!h]
\setcounter{algorithm}{1}
\caption{AC-\textsc{Dibs}}
\label{alg:ac_dibs_alg}
\textsc{Input:} $\pi_d, M, \beta, \Delta, \epsilon, \text{{\it rounds}}, \text{{\it iters}}$ \\
\textsc{Output}: $\phi, \pi_\phi$

\begin{algorithmic}[1]

% Initialize.
\State{$\forall_{s} : \phi^{(0)}(s) = \texttt{random.choice}([1,|\mc{S}|])$} \Comment{Initialize}
\State{$\forall_{s} : \pi_{\phi}^{(0)}(a \mid s_\phi) \sim \mathrm{Unif}(\mc{A})$}
\State{$\rho_\phi^{(0)} \la \texttt{get\_stationary\_pmf}(M, \pi_{\phi}^{(0)}, \phi^{(0)})$}

% Iterative Updates.
\For{$\text{i} = 1$ to $\text{{\it rounds}}$} 

    \State{$\pi_\phi^{(i)}, \phi^{(i)} = \textsc{Dibs}(\pi_d, \rho_\phi^{(i-1)}, M, \beta, \Delta, \text{{\it iters}})$}
    
    \State{$\rho_\phi^{(i)}(s) = \texttt{get\_stationary\_pmf}(M, \pi_\phi^{(i)}, \phi^{(i)})$}
    
    %\State{}\Comment{Check convergence}
    \If{$\mathrm{L_1}\left(\rho_\phi^{(i-1)}, \rho_\phi^{(i)}\right) \leq \epsilon$} 
        \State{\texttt{break}} \Comment{Converged}
    \EndIf
    
\EndFor \\
\Return{$\phi_{t+1}, \pi_{\phi,t+1}$}
\end{algorithmic}
\label{alg:ac_dibs}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%

==> misc/contrib_old_table.tex <==

\begin{center}
    \textbf{State Abstraction} (\autoref{part:state_abstraction})
\end{center}
% C2: Approx SA

\begin{center}
\begin{tabular}{cc}%{p{1.5cm}p{1.5cm}}
% Approximate State Abstr.
    \multicolumn{2}{c}{\it Approximate State Abstraction} (\autoref{chap:approx_state_abstr}) \\
     Question&Answer \\
     
     \multicolumn{2}{c}{\it State Abstractions for Lifelong RL} (\autoref{chap:state_abstr_lifelong}) \\
     Question&Answer \\
     
     \multicolumn{2}{c}{\it State Abstraction As Compression in Apprenticeship Learning} (\autoref{chap:rlit}) \\
     Question&Answer \\
\end{tabular}
\end{center}


\midrule


\begin{center}
    \textbf{Action Abstraction}
\end{center}
% C2: Approx SA

\begin{center}
\begin{tabular}{cc}%{p{1.5cm}p{1.5cm}}
% Approximate State Abstr.
    \multicolumn{2}{c}{\it Finding Options that Minimize Planning Time} (\autoref{chap:options_for_planning}) \\
     Question&Answer \\
     
     \multicolumn{2}{c}{\it The Expected-Length Model of Options} (\autoref{chap:elm_options}) \\
     Question&Answer \\
     
     \multicolumn{2}{c}{\it Discovering Options for Exploration} (\autoref{chap:options_for_exploration}) \\
     Question&Answer \\
\end{tabular}
\end{center}



\midrule


\begin{center}
    \textbf{State-Action Abstraction}
\end{center}
% C2: Approx SA



% \dbox{\textbf{Summary of Contributions}: \\

%     {\it State Abstraction}
%     \begin{itemize}
%     % State abstraction chapters
%         \item[$\rightslice$] Framework for approximate state abstraction that preserve near-optimal behavior in arbitrary MDPs~\cite{abel2016near}.
%         \item[$\rightslice$] Characterizing and computing state abstractions for lifelong RL that preserve near-optimal behavior~\cite{abel2018salrl}.
%         %\item[$\rightslice$] Learning policies/value functions for lifelong RL~\cite{abel2018transfer}.

%         \item[$\rightslice$] Information theoretic view for understanding abstraction as compression.
%     \end{itemize}
    
%     % Options chapters
%     {\it Action Abstraction}
%     \begin{itemize}
%         \item[$\rightslice$] Expected-Length Model of Options
%         \item[$\rightslice$] Characterizing the computational complexity of finding options that minimize planning time, and an approximation algorithm.
        
%         \item[$\rightslice$] Proposal of new algorithm for discovering options that accelerate exploration.
        
%         {\it Hierarchical Abstraction}
%         \item[$\rightslice$] Computing action abstractions/hierarchies from state abstractions.
% \end{itemize}}


==> misc/contributions_one_pager.tex <==

%%%%%%%
% Part 2
\noindent
\begin{minipage}[t]{.5\textwidth}
\begin{center}
    \hypersetup{hidelinks}
    %\textbf{Part 2} \\
    \textbf{\autoref{part:state_abstraction}}
    
    \textcolor{partred}{STATE ABSTRACTION}
\end{center}
%%% PART 2 CONTENT HERE

%%%
\end{minipage}% <---------------- Note the use of "%"
\begin{minipage}[t]{.5\textwidth}
\begin{center}
    \hypersetup{hidelinks}
    \textbf{\autoref{part:action_abstraction}} \\
    
    \textcolor{partred}{ACTION ABSTRACTION}
\end{center}
\end{minipage}


%%%%%%%
% Part 1
\begin{center}
    \hypersetup{hidelinks}
    \textbf{\autoref{part:state_action_abstraction}} \\
    
    \normalsize{\textcolor{partred}{STATE-ACTION ABSTRACTION}}
\end{center}

==> misc/grid_mdp_defs.tex <==
\begin{enumerate}
%
\item States.
$\mc{S} = \{(1,1), (2,1), (3,1), (4,1), (1,2), (3,2), (4,2), (1,3), (2,3), (3,3), (4,3)\}$
%
\item Actions.
$\mc{A} = \{\uparrow,\ \ra,\ \downarrow,\ \la\}$
%
\item Rewards.
$R(s,a,s') = \begin{cases}
1& s' = (4,3), \\
-1& s' = (4,2), \\
0& \text{otherwise}, \\
\end{cases}$
%
\item Transitions.
$T(s' \mid s,a) = \indic\{s' = \texttt{grid\_\hspace{1pt}move}(s,a)\}$
where,
\[
\texttt{grid\_\hspace{1pt}move}(s ,a) = \begin{cases}
%\texttt{end\_\hspace{1pt}episode}& s \in \{(4,3), (4,2)\} \\
(s.x, \min(s.y + 1, 3)) &a =\ \uparrow \text{and}\ s.x \neq 2,\\
(\min(s.x + 1, 4), s,y)  &a =\ \ra \text{and}\ s \neq (1,2),\\
(s.x, \max(s.y - 1, 1)) &a =\ \downarrow \text{and}\ s.x \neq 2,\\
(\max(s.x - 1, 1), s,y) &a =\ \la \text{and}\ s \neq (3,2),\\
s& \text{otherwise}
\end{cases}
\]
%
\item Start distribution.
$\rhoz(s) = \indic\{s = (1,1)\}$
%
\item Discount factor.
$\gamma = 0.99.$
\end{enumerate}

==> preface/fancy_title_page.tex <==
\begin{titlepage} % Suppresses displaying the page number on the title page and the subsequent page counts as page 1
	\newcommand{\HRule}{\rule{\linewidth}{0.5mm}} % Defines a new command for horizontal lines, change thickness here
	
	\center % Centre everything on the page
	
	%------------------------------------------------
	%	Headings
	%------------------------------------------------
	
	\textsc{\Large Brown University}\\[0.5cm] % Main heading such as the name of your university/college
	
	\textsc{\Large Department of Computer Science}\\[0.5cm] % Major heading such as course name
	
	%\textsc{\large Ph.D Thesis Proposal}\\[0.5cm] % Minor heading such as course title
	
	\vspace{50mm}

	%------------------------------------------------
	%	Title
	%------------------------------------------------
	
	%\HRule\\[0.4cm]
	
	\rule{\textwidth}{1.6pt}\vspace*{-\baselineskip}\vspace*{2pt} % Thick horizontal rule
	\rule{\textwidth}{0.4pt} % Thin horizontal rule
	
	\vspace{0.75\baselineskip} % Whitespace above the title
	
	{\LARGE Effective Reinforcement Learning through State Abstraction\\}
	%{\LARGE The Role of State Abstraction in Reinforcement Learning\\} % Title
	%{\fontsize{19pt}{20pt}\selectfont The Role of State Abstraction in Reinforcement Learning\\}
	
	\vspace{0.75\baselineskip} % Whitespace below the title
	
	\rule{\textwidth}{0.4pt}\vspace*{-\baselineskip}\vspace{3.2pt} % Thin horizontal rule
	\rule{\textwidth}{1.6pt} % Thick horizontal rule
	
	\vspace{2\baselineskip} % Whitespace after the title block
	
	
	%------------------------------------------------
	%	Author(s)
	%------------------------------------------------
	
	\begin{minipage}{0.4\textwidth}
		\begin{flushleft}
			\large
			\textit{Author}\\
			David Abel
		\end{flushleft}
	\end{minipage}
	~
	\begin{minipage}{0.4\textwidth}
		\begin{flushright}
			\large
			\textit{Doctoral Advisor}\\
			Dr. Michael L. Littman % Supervisor's name
		\end{flushright}
	\end{minipage}
	
	\vspace{20mm}
	
	
	
	%------------------------------------------------
	%	Date
	%------------------------------------------------
	
	\textsc{\large Ph.D Thesis}\\[0.5cm]
	
	\vfill\vfill\vfill % Position the date 3/4 down the remaining page
	
	{\large May 2020} % Date, change the \today to a set date if you want to be precise
	
	
	%------------------------------------------------
	%	Logo
	%------------------------------------------------
	
	\vfill\vfill
	\includegraphics[width=0.2\textwidth]{figures/diagrams/brown.pdf}\\[1cm] % Include a department/university logo - this will require the graphicx package
	 
	%----------------------------------------------------------------------------------------
	
	\vfill % Push the date up 1/4 of the remaining page
	
\end{titlepage}

==> preface/sig_two.tex <==
\begin{tabular}{lc}
      Date \rule{1in}{.05mm}\hspace*{.75in} & \rule{3in}{.05mm}\\
      & ##1\\ & ##2
\end{tabular}
 \null\vskip.2in

==> proofs/c6/c6_mimo_momi_np_hard.tex <==
\begin{dproof}[Theorem \ref{thm:c6_mimo_momi_np-hard}]
    % TODO: reduction
    To prove the theorem, let us consider OI-DEC, a decision problem variant of MIMO and MOMI. This problem asks if we can solve the MDP within $\ell$ iterations using at most $k$ point options.
    
    %\ddef{OI-DEC}{ \\
    \begin{definition}
        The \textbf{OI-DEC} problem is defined as follows: \texttt{given} an MDP $M$, a non-negative real-value $\epsilon$,  and integers $k$ and $\ell$, \texttt{return} `Yes' if the there exists an option set $\mc{O}$ such that $\mc{O} \subseteq \mc{O}_p$, $|\mc{O}| \leq k$ and $L(\mc{O}) \leq \ell$. `No' otherwise.
    \end{definition}
    
    The proof proceeds by reduction from the decision version of the set-cover problem---known to be NP-complete---to OI-DEC. The set-cover problem is defined as follows.

    %\ddef{SetCover-DEC} { \\
    \begin{definition}
        The \textbf{SetCover-DEC} problem is defined as follows: \texttt{given} a set of elements $\mc{U}$, a set of subsets $\mc{X} = \{X \subseteq \mc{U}\}$, and an integer $k$, \texttt{return} `Yes' if there exists a cover $\mc{C} \subseteq \mc{X}$ that $\bigcup_{X \in \mc{C}} X = \mc{U}$ and $|\mc{C}| \leq k$. `No' otherwise.
    %}
    \end{definition}
    
    If there is some $u \in \mc{U}$ that is not included in at least one of the subsets $X$, then the answer is `No'.
    
    Assuming otherwise, we construct an instance of a shortest path problem (a special case of an MDP problem) as follows (\autoref{fig:c6_sdec_oidec}).
    There are four types of states in the MDP: (1) $u_i \in \mc{U}$ represents one of the elements in $\mc{U}$, (2) $X_i \in \mc{X}$ represents one of the subsets in $\mc{X}$, (3) $X'_i \in \mc{X}'$: we make a copy for every state $X_i \in \mc{X}$ and call them $X'_i$, (4) a goal state $g$.
    Thus, the state set is $\mc{U} \cup \mc{X} \cup \mc{X}' \cup \{g\}$.
    We build edges between states as follows:
    (1) $e(u, X) \in E$ iff $u \in X$: For $u \in \mc{U}$ and $X \in \mc{X}$, there is an edge between $u$ and $X$.
    (2) $\forall X_i \in \mc{X}$, $e(X_i, X'_i) \in E$: For every $X_i \in \mc{X}$, we have a edge from $X_i$ to $X'_i$. (3) $\forall e(X', g) \in E$: for every $X' \in \mc{X}'_i$ we have a edge from $X_i$ to the goal $g$.
    This construction can be done in polynomial time. % linear time?

    Let $M$ be the MDP constructed in this way.
    We show that SetCover($\mc{U}, \mc{X}, k$) = OI-DEC($M, k, 2$).
    Note that by construction every state $s_i$, $s'_i$, and $g$ converges to its optimal value within 2 iterations as it reaches the goal state $g$ within 2 steps. A state
    $u \in \mc{U}$ converges within 2 steps if and only if there exists a point option (a) from $X$ to $g$ where $u \in X$, (b) from $u$ to $X'$ where $u \in X$, or (c) from $u$ to $g$. For options of type (b) and (c), we can find an option of type (a) that makes $u$ converge within 2 steps by setting the initial state of the option to $\mc{I}_o = X$, where $u \in X$, and the termination state to $\beta_o = g$.
    % Then every $x \in X$ converges within 2 steps if we set options from $s$ to $g$ so that for every $x$ there exists $s$ such that $x \in s$.
    Let $\mc{O}$ be the solution of OI-DEC($M, k, 2$).
    If there exists an option of type (b) or (c), we can swap them with an option of type (a) and still maintain a solution.
    Let $\mc{C}$ be a set of initial states of each option in $\mc{O}$ ($\mc{C} = \{\mc{I}_o \mid o \in \mc{O}\}$).
    This construction exactly matches the solution of the SetCover-DEC.
    
\end{dproof}

==> proofs/c6/c6_mom_hard_approx_ONE.tex <==
\begin{proof}%[Condition 1.]
    The optimization version of the set-cover problem cannot be approximated within a factor of $c \cdot \ln n$ by a polynomial-time algorithm unless P = NP~\cite{raz1997sub}. The set-cover optimization problem can be reduced to MOMI with a similar construction for a reduction from SetCover-DEC to OI-DEC. Here, the targeted minimization values of the two problems are equal: $P(\mc{C}) = |\mc{O}|$, and the number of states in OI-DEC is equal to the number of elements in the set cover on transformation.
    
    Assume there is a polynomial-time algorithm within a factor of $c \cdot \ln n$ approximation for MOMI where $n$ is the number of states in the MDP.
    Let SetCover$(\mc{U}, \mc{X})$ be an instance of the set-cover problem. We convert the instance into an instance of MOMI$(M, 0, 2)$.
    Using the approximation algorithm, we get a solution $\mc{O}$ where $|\mc{O}| \leq c \ln n |\mc{O}^*|$, where $\mc{O}^*$ is the optimal solution.
    
    We construct a solution for the set cover $\mc{C}$ from the solution to the MOMI $\mc{O}$ (see the construction in the proof of \autoref{thm:c6_mimo_momi_np-hard}).
    Because $|\mc{C}| = |\mc{O}|$ and $|\mc{C}^*| = |\mc{O}^*|$, where $\mc{C}^*$ is the optimal solution for the set cover, we get $|\mc{C}| = |\mc{O}| \leq c \ln n |\mc{O}^*| = c \ln n |\mc{C}^*|$. Thus, we acquire a $c \cdot \ln n$ approximation solution for the set-cover problem within polynomial time, which is possible if P=NP.
    
    Thus, there is no polynomial-time algorithm with a factor of $c \cdot \ln n$ approximation for MOMI, unless P=NP.
\end{proof}

==> proofs/c6/c6_mom_hard_approx_THREE.tex <==
\begin{proof}%[Lemma \ref{lem:c6_momi_hard_approx_THREE}]
Assume $\text{NP} \not \subseteq \text{DTIME}(n^ {\poly \log n})$ and for the sake of contradiction that there exists an $\eps > 0$ for which a polynomial-time algorithm $\mc{A}_\momi$ can $2^{\log^{1 - \eps} n }$-approximate \momi. We use $\mc{A}_\momi$ to $2^{\log^{1 - \eps'} \tilde{n}}$ approximate Min-Rep for a fixed constant $\eps' > 0$ in polynomial-time in $\tilde{n}$, thereby contradicting \autoref{lem:minRepHard}. Again, $\tilde{n}$ is the number of vertices in the graph of the Min-Rep instance.

We begin by noting that the relevant quantities in $\momi(\MR)$ are polynomially-bounded. Let $\tilde{n} := |A| + |B|$ be the number of vertices in our \MR instance. Notice that the number of states in the MDP, $n$, in our $\momi(\MR)$ instance is at most $O(\tilde{n} + 2|A||\Sigma_A|  + |B||\Sigma_B| + |E|) \leq \tilde{n}^c$ for some fixed constant $c$ by the aforementioned assumption that $\Sigma_A$ and $\Sigma_B$ are polynomially-bounded in $\tilde{n}$.\footnote{It is worth noting, also, that since we create at most $\sum_e |\pi_e|$ actions for any state, the number of total actions in our MDP is at most polynomial in $\tilde{n}$.}

Our polynomial-time approximation algorithm to approximate instance \MR of Min-Rep is as follows: Run $\mc{A}_\momi$ on $\momi(\MR)$ to get back option set $\mc{O}$. Return $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$ as defined above as our solution to \MR.

We first argue that our algorithm is polynomial time in $\tilde{n}$. For each vertex in \MR, we create a polynomial number of states and actions. Thus, the number of states in $\momi(\MR)$ is polynomially-bounded in $\tilde{n}$ and so $\mc{A}_\momi$ runs in time polynomial in $\tilde{n}$. A polynomial runtime of our algorithm immediately follows.

We now argue that our algorithm is a $2^{\log^{1 - \eps'} \tilde{n} }$-approximation for Min-Rep for some $\eps' > 0$. Applying Lemma 3 from \citet{jinnai2019opt}, the approximation of $\mc{A}_\momi$, and then Lemma 4 from \citet{jinnai2019opt}, we have that the Min-Rep cost of $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$ is
%Applying \autoref{lem:MRToMomiStoch}, the approximation of $\mc{A}_\momi$ and then \autoref{lem:MRRelateOpt}, we have that the Min-Rep cost of $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$ is
\begin{align*}
\cost_{\text{Min-Rep}}(\gamma^\mc{O}_A, \gamma^\mc{O}_B) & = |\mc{O}|\\ &\leq 2^{\log^{1-\eps} n } \OPT_\momi \\
&\leq 2^{\log^{1-\eps} n } \OPT_\MR
\end{align*}

Thus, $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$ is a $2^{\log^{1-\eps}n}$ approximation for the optimal Min-Rep solution where $n$ is the number of states in the MDP of $\momi(\MR)$. Now recalling that $n \leq \tilde{n}^c$ for fixed constant $c$. We therefore have that $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$ is a $2^{\log^{1-\eps} \tilde{n}^c} = 2^{c^{1- \eps} \log^{1-\eps} \tilde{n}} \leq c' \cdot 2^{ \log^{1-\eps} \tilde{n}}$ approximation for a constant $c'$. Choosing $\eps$ sufficiently small, we have that $c' \cdot 2^{ \log^{1-\eps} \tilde{n}} \leq 2^{ \log^{1-\eps'} \tilde{n}}$ for sufficiently large $\tilde{n}$. 

Thus, our polynomial-time algorithm is a $2^{\log^{1 - \eps'} \tilde{n} }$-approximation for Min-Rep for $\eps' > 0$, thereby contradicting \autoref{lem:minRepHard}. We conclude that \momi cannot be $2^{\log^{1- \epsilon} n}$-approximated.
\end{proof}

==> proofs/c6/c6_mom_hard_approx_TWO.tex <==
\begin{proof}%[Lemma \ref{lem:c6_momi_hard_approx_TWO}]
Assume $\text{NP} \not \subseteq \text{DTIME}(n^ {\poly \log n})$ and for the sake of contradiction that there exists an $\eps > 0$ for which polynomial-time algorithm $\mc{A}_{\momichoose}$ can $2^{\log^{1 - \eps} n }$-approximate \momichoose. We use $\mc{A}_{\momichoose}$ to $2^{\log^{1 - \eps'} \tilde{n}}$ approximate Min-Rep for a fixed constant $\eps' > 0$ in polynomial-time, thereby contradicting \autoref{lem:minRepHard}. Again, $\tilde{n}$ is the number of vertices in the graph of the Min-Rep instance.

We begin by noting that the relevant quantities in $\momichoose(\MR)$ are polynomially-bounded. Notice that the number of states $n$ in the MDP in $\momichoose(\MR)$ is at most $O(\tilde{n}^2 |\Sigma_A| |\Sigma_B|) = \tilde{n}^c$ for some fixed constant $c$ by the aforementioned assumption that $\Sigma_A$ and $\Sigma_B$ are polynomially-bounded in $\tilde{n}$.\footnote{It is also worth noticing that since we create at most $O(\tilde{n}|\Sigma_A| + \tilde{n}|\Sigma_B|)$ options, the total number of options in $\mc{O}'$ is at most polynomial in $\tilde{n}$.}

Our polynomial-time approximation algorithm to approximate instance \MR of Min-Rep is as follows: Run $\mc{A}_{\momichoose}$ on $\momichoose(\MR)$ to get back option set $\mc{O}$. Return $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$ as defined above as our solution to \MR.

We first argue that our algorithm is polynomial-time in $\tilde{n}$. However, notice that for each vertex, we create a polynomial number of states. Thus, the number of states in $\momichoose(\MR)$ is polynomially-bounded in $\tilde{n}$ and so $\mc{A}_{\momichoose}$ runs in time polynomial in $\tilde{n}$. A polynomial runtime of our algorithm immediately follows.

We now argue that our algorithm is a $2^{\log^{1 - \eps'} \tilde{n} }$-approximation for Min-Rep for some $\eps' > 0$. Applying Lemma 3 by \citet{jinnai2019opt}, the approximation of $\mc{A}_{\momichoose}$, and then Lemma 2 by \citet{jinnai2019opt}, we have that $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$  is a feasible solution for \MR with cost
\begin{align}
\cost_{\text{Min-Rep}}(\gamma^\mc{O}_A, \gamma^\mc{O}_B) & = |\mc{O}|\\ &\leq 2^{\log^{1-\eps} n } \OPT_{\momichoose} \\
&\leq 2^{\log^{1-\eps} n } \OPT_\MR.
\end{align}

Thus, $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$ is a $2^{\log^{1-\eps}n}$ approximation for the optimal Min-Rep solution where $n$ is the number of states in the MDP of $\momichoose(\MR)$. Now recalling that $n \leq \tilde{n}^c$ for fixed constant $c$. We therefore have that $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$ is a $2^{\log^{1-\eps} \tilde{n}^c} = 2^{c^{1- \eps} \log^{1-\eps} \tilde{n}} \leq c' \cdot 2^{ \log^{1-\eps} \tilde{n}}$ approximation for a constant $c'$. Choosing $\eps$ sufficiently small, we have that $c' \cdot 2^{ \log^{1-\eps} \tilde{n}} \leq 2^{ \log^{1-\eps'} \tilde{n}}$ for sufficiently large $\tilde{n}$. 

Thus, our polynomial-time algorithm is a $2^{\log^{1 - \eps'} \tilde{n} }$-approximation for Min-Rep for $\eps' > 0$, thereby contradicting \autoref{lem:minRepHard}. We conclude that \momichoose cannot be $2^{\log^{1- \epsilon} n}$-approximated.
\end{proof}

==> proofs/c6/c6_momi_hard_approx.tex <==
\begin{dproof}[Theorem \ref{thm:c6_MOMIHardness}]
The proof strategy is divided amongst each of the three cases. I offer these proofs in three independent arguments as follows.

% Probably need some extra details here.

% Lemma 6.4.1
\begin{lemma}
    MOMI is $\Omega(\log n)$ hard to approximate even for deterministic MDPs unless P = NP.
    \label{lem:c6_momi_hard_approx_ONE}
\end{lemma}
\input{proofs/c6/c6_mom_hard_approx_ONE}
\spacerule

For the next two lemmas we reduce our problem to the Min-Rep problem originally defined by \citet{kortsarz2001hardness}. Min-Rep is a variant of the better studied label cover problem \cite{dinur2004hardness} and has been integral to recent hardness of approximation results in network design problems \cite{dinitz2012label,bhattacharyya2012transitive}. Roughly, Min-Rep asks how to assign as few labels as possible to nodes in a bipartite graph such that every edge is ``satisfied.'' 

\begin{definition}
The \textbf{Min-Rep} problem is defined as follows {\bf given} a bipartite graph $G = (A \cup B, E)$ and alphabets $\Sigma_A$ and $\Sigma_B$ for the left and right sides of $G$ respectively. Each $e \in E$ has associated with it a set of pairs $\pi_{e} \subseteq \Sigma_A \times \Sigma_B$ which satisfy it. {\bf Return} a pair of assignments $\gamma_A : A \to \mc{P}(\Sigma_A)$ and $\gamma_B : B \to \Delta(\Sigma_B)$ such that for every $e=(A_i,B_j) \in E$  there exists an $(a, b) \in \pi_e$ such that $a \in \gamma_A(A_i)$ and $b \in \gamma_B(B_j)$. The objective is to minimize $\sum_{A_i \in A} |\gamma_A(A_i)| + \sum_{B_j \in B} |\gamma_B(B_j)|$.
\end{definition}
\definecolor{OptionColor1}{HTML}{4285F4}
\definecolor{OptionColor2}{HTML}{FBBC05}
\definecolor{OptionColor3}{HTML}{34A853}
\definecolor{OptionColor4}{HTML}{EA4335}
\definecolor{OptionColor5}{HTML}{4F6367}
\definecolor{OptionColor6}{HTML}{D138BF}
\definecolor{OptionColor7}{HTML}{7494EA}

\tikzstyle{MREdgeStyle}=[thick, sloped]
\tikzstyle{SatAssignmentNode}=[color=OptionColor1]
\tikzstyle{MRNodeStyle}=[draw, circle, thick, minimum size=1cm]
\usetikzlibrary{positioning}

% We illustrate a feasible solution to an instance of Min-Rep in \Cref{fig:minrep}. 
% \begin{figure}[hb]
%     \centering
%     \begin{tikzpicture}
%     % A
%     \node [MRNodeStyle] (A1) at (0, 4) {$A_1$};
%     \node [MRNodeStyle] (A2) at (0, 2) {$A_2$};
%     % B 
%     \node [MRNodeStyle] (B1) at (3, 4) {$B_1$};
%     \node [MRNodeStyle] (B2) at (3, 2) {$B_2$};
        
%     % E
%     \draw[MREdgeStyle] (A1) -- (B1)  node[midway, above] {\tiny \color{OptionColor2} $(a_1, b_2)$};
%     \draw[MREdgeStyle] (A1) -- (B2) node[midway, above] {\tiny \color{OptionColor3} $(a_2, b_3)$, \color{OptionColor4} $(a_3, b_1)$};
%     \draw[MREdgeStyle] (A2) -- (B2) node[midway, above] {\tiny \color{OptionColor5} $(a_3, b_1)$};
    
%     %Sat assignment
%     \node [SatAssignmentNode, below=0cm of A1] {$a_1, a_2$};
%     \node [SatAssignmentNode, below=0cm of A2] {$a_3$};
%     \node [SatAssignmentNode, below=0cm of B1] {$b_2$};
%     \node [SatAssignmentNode, below=0cm of B2] {$b_1, b_3$};
    
%     \end{tikzpicture}
%     \caption{An instance of Min-Rep with $\Sigma_A = \{a_1, a_2, a_3\}$ and $\Sigma_B = \{b_1, b_2, b_3\}$. Edge $e$ is labeled with pairs in $\pi_e$. Feasible solution $(\gamma_A, \gamma_b)$ illustrated where $\gamma_A(A_i)$ and $\gamma_B(B_j)$ below $A_i$ and $B_j$ in blue. Constraints colored to coincide with stochastic action colors in \Cref{fig:minrepstochMOMIred}.}
%     \label{fig:minrep}
% \end{figure}

The crucial property of Min-Rep we use is that no polynomial-time algorithm can approximate Min-Rep well. 
Let $\tilde{n} = |A| + |B|$.
\begin{lemma}[\citeauthor{kortsarz2001hardness} \citeyear{kortsarz2001hardness}]\label{lem:minRepHard}
Unless $\text{NP} \subseteq \text{DTIME}(n^ {\poly \log n})$, Min-Rep admits no $2^{\log^{1 - \eps} \tilde{n}}$ polynomial-time approximation algorithm for any $\eps > 0$.
\end{lemma}
As a technical note, note that all relevant quantities in Min-Rep are polynomially-bounded. In Min-Rep we have $|\Sigma_A|, |\Sigma_B| \leq \tilde{n}^{c'}$ for constant $c'$. It immediately follows that $\sum_e |\pi_e| \leq n^c$ for constant $c$.

% We now show that a solution to $\momichoose(\MR)$ corresponds to a solution to \MR. For the remainder of this section $\gamma^\mc{O}_A(A_i) : = \{a : O(A_i,a) \in \mc{O} \}$ and $\gamma^\mc{O}_B(B_j) : = \{b : O(B_j,b) \in \mc{O} \}$ is the Min-Rep solution corresponding to option set $\mc{O}$.
% \begin{lemma}\label{lem:MRToMomiChoose}
% For a feasible solution to $\momichoose(\MR)$, $\mc{O}$, we have $(\gamma^\mc{O}_A, \gamma^\mc{O}_B)$ is a feasible solution to \MR of cost $|\mc{O}|$.
% \end{lemma}

% \begin{proof}
% Notice that by construction the Min-Rep cost of $(\gamma^{\mc{O}}_A, \gamma^{\mc{O}}_B)$ is exactly $|\mc{O}|$. Thus, we need only prove that $(\gamma^{\mc{O}}_A, \gamma^{\mc{O}}_B)$ is a feasible solution for \MR. 

% We do so now. Consider an arbitrary edge $e = (A_i, B_j) \in E$; we wish to show that $(\gamma^{\mc{O}}_A, \gamma^{\mc{O}}_B)$ satisfies $e$. Since $\mc{O}$ is a feasible solution to $\momichoose(\MR)$ we know that after 3 iterations of value iteration every state must converge on its value. Moreover, notice that the value of every state in $\momichoose(\MR)$ is $1$. Thus, it must be the case that for every $S_e$ there exists a path of length 3 from $S_e$ to $S_g$ using either options or actions. The only such paths are those that take an option $O(A_i, a)$, then an action from $S_{ea}$ to $S_{eb}$ then option $O(B_j, b)$ where $(a, b) \in \pi_e$. It follows that $a \in \gamma^{\mc{O}}_A(A_i)$ and $b \in \gamma^{\mc{O}}_B(B_j)$. But since $(a, b) \in \pi_e$, we then know that $e$ is satisfied. Thus, every edge is satisfied and so $(\gamma^{\mc{O}}_A, \gamma^{\mc{O}}_B)$ is a feasible solution to \MR.
% \end{proof}

With Min-Rep in place, let us not turn to the other two lemmas that prove the theorem.

% Lemma 6.4.2
\begin{lemma}
    MOMI$_{gen}$ is $2^{\log^{1-\epsilon}n}$-hard to approximate for any $\epsilon>0$ even for deterministic MDP unless $\text{NP} \subseteq \text{DTIME}(n^{poly \log n})$.
    \label{lem:c6_momi_hard_approx_TWO}
\end{lemma}
\input{proofs/c6/c6_mom_hard_approx_TWO}
\spacerule

% Lemma 6.4
\begin{lemma}
    Unless NP $\subseteq$ DTIME$(n^{poly \log n})$, MOMI is $2^{\log^{1-\epsilon}n}$-hard to approximate for any $\epsilon>0$.
    \label{lem:c6_momi_hard_approx_THREE}
\end{lemma}
\input{proofs/c6/c6_mom_hard_approx_THREE}

\end{dproof}


==> proofs/c8/c8_cover_time_value.tex <==
\begin{dproof}[Theorem \ref{thm:c8_value_cover_time}]
    The value of state $s$ is $r_c$ times the expected number of steps to reach the goal state. Thus, 
    \begin{align}
        V_g^\pi(s) &= r_c \bE[ H_{sg} ] \\
                &\geq r_c \bE[ \max_{s' \in S} H_{ss'} ] \\
                &= r_c \bE[ C_s(G) ] \\
                &\geq r_c \bE[ C(G) ].
    \end{align}
\end{dproof}

==> proofs/c8/c8_options_cover_time.tex <==
\begin{dproof}[Theorem \ref{thm:c8_option_cover_time}]
    Assume the multiplicity of the second smallest eigenvalue is one. Let $\mathcal{L}'$ be the graph Laplacian of the graph with an edge inserted to $\mathcal{L}$ using the algorithm by \citet{ghosh2006growing}.
    By adding a single edge, the algebraic connectivity is guaranteed to increase at least by $F$:
    \begin{equation}
        \lambda_2 \geq \lambda_2 + \frac{(v_i - v_j)^2}{6 / (\lambda_3 - \lambda_2) + 3 / 2},
    \end{equation}
    and the upper bound of the cover time is guaranteed to decrease:
    \begin{align}
        \bE[C(G')] &\leq \frac{n^2 \ln n}{\lambda_{2}} (1 + o(1)) \\
        &\leq \frac{n^2 \ln n}{\lambda_{2} + \frac{(v_i - v_j)^2}{6 / (\lambda_3 - \lambda_2) + 3 / 2}} (1 + o(1)).
    \end{align}
    As $\frac{(v_i - v_j)^2}{6 / (\lambda_3 - \lambda_2) + 3 / 2}$ is positive,
    \begin{equation}
        \frac{n^2 \ln n}{\lambda_{2} + \frac{(v_i - v_j)^2}{6 / (\lambda_3 - \lambda_2) + 3 / 2}} (1 + o(1)) < \frac{n^2 \ln n}{\lambda_{2}} (1 + o(1)),
    \end{equation}
    thus the upper bound is guaranteed to decrease.
\end{dproof}

==> proofs/option_kappa_estimate.tex <==
\begin{dproof}
For a fixed but arbitrary state--option--state triple $(s,o,s')$, let $\kappa$ denote $\kappa_s^o$, and by assumption let $h = \frac{1}{1-\gamma}$ be the maximum number of steps taken by an option:
\begin{align}
    \mc{T}_\gamma(s,o,s') - \mc{T}_\kappa(s,o,s') &= \sum_{t=1}^{h} \gamma^t \Pr(s_t = s', \beta(s_t) \mid s, o) - \gamma^\kappa \sum_{t=1}^{h} \Pr(s_t = s', \beta(s_t) \mid s, o) \\
    &= \sum_{t=1}^{h} (\gamma^t \Pr(s_t = s', \beta(s_t) \mid s, o) - \gamma^\kappa \Pr(s_t = s', \beta(s_t) \mid s, o)) \\
    &= \sum_{t=1}^{h} (\gamma^t - \gamma^\kappa) \Pr(s_t = s', \beta(s_t) \mid s, o) \\
    &= \sum_{t=1}^{h} (\gamma^t - \gamma^\kappa) \Pr(s_t = s' \mid s, o) \cdot \Pr(\beta(s_t))
\end{align}

Note that $\Pr(s_t = s' \mid s, o)$ is bounded above:
\begin{equation}
    \Pr(s_t, = s' \mid s, o) \leq (1 - \beta_{\min})^t,
\end{equation}
since, to be in state $s_t$ at time $t$, we have to {\it not} terminate in each of $s_1, \ldots s_t$. Further, we know that:
\begin{equation}
    (1-x)^t \leq e^{-xt}
\end{equation}
for any $x \in [0,1]$. Therefore:
\begin{equation}
\Pr(s_t, = s' \mid s, o) \leq e^{-\beta_{\min}t}.
\end{equation}

So, rewriting:
\begin{align}
    \mc{T}_\gamma(s,o,s') - \mc{T}_\kappa(s,o,s') &= \sum_{t=1}^{h} (\gamma^t - \gamma^\kappa) \Pr(s_t = s' \mid s, o) \cdot \Pr(\beta(s_t)) \\
%    & \leq \sum_{t=1}^{h} (\gamma^t - \gamma^\kappa) e^{-\beta_{\min}t} \\
    & \leq \sum_{t=1}^{h} (\gamma^t - \gamma^\kappa) e^{-\beta_{\min}t}. \label{eq:has_negative}
\end{align}
But, note that when $t \leq \kappa$, for any $\beta_{\min} \in [0,1]$:
\begin{equation}
(\gamma^t - \gamma^\kappa) e^{-\beta_{\min}t} \leq 0.    
\end{equation}

Therefore:
\begin{align}
    \mc{T}_\gamma(s,o,s') - \mc{T}_\kappa(s,o,s') &\leq \sum_{t=1}^{h} (\gamma^t - \gamma^\kappa) e^{-\beta_{\min}t}\\
    &\leq \sum_{j=1}^{h-\kappa} (\gamma^{j + \kappa} - \gamma^\kappa) e^{-\beta_{\min}(j + \kappa)} \\
    &= \sum_{j=1}^{h-\kappa} (\gamma^j \gamma^\kappa - \gamma^\kappa) e^{-\beta_{\min} (j + \kappa)} \\
    &= \sum_{j=1}^{h-\kappa} \gamma^\kappa (\gamma^j - 1) e^{-\beta_{\min} (j + \kappa)} \\
    &\leq \sum_{j=1}^{h-\kappa} \gamma^\kappa e^{-\beta_{\min} (j + \kappa)}.
\end{align}
Since $0 \leq e^{-x} \leq 1$ for $x \geq 0$, we conclude:
\begin{align}
    \mc{T}_\gamma(s,o,s') - \mc{T}_\kappa(s,o,s') &\leq  \sum_{j=1}^{h-\kappa} \gamma^\kappa e^{-\beta_{\min} (j + \kappa)} \\
    &\leq (h-\kappa) \gamma^\kappa e^{-\beta_{\min} \kappa}. \qedhere
\end{align}
\end{dproof}
%%%%%%%%%%%%%%%%%%
